Measuring justice in machine learning

How can we build more just machine learning systems? To answer this question, we need to know both what justice is and how to tell whether one system is more or less just than another. That is, we need both a definition and a measure of justice. Theories of distributive justice hold that justice can be measured (in part) in terms of the fair distribution of benefits and burdens across people in society. Recently, the field known as fair machine learning has turned to John Rawls's theory of distributive justice for inspiration and operationalization. However, philosophers known as capability theorists have long argued that Rawls's theory uses the wrong measure of justice, thereby encoding biases against people with disabilities. If these theorists are right, is it possible to operationalize Rawls's theory in machine learning systems without also encoding its biases? In this paper, I draw on examples from fair machine learning to suggest that the answer to this question is no: the capability theorists' arguments against Rawls's theory carry over into machine learning systems. But capability theorists don't only argue that Rawls's theory uses the wrong measure, they also offer an alternative measure. Which measure of justice is right? And has fair machine learning been using the wrong one?

==> _abstractpage.tex <==
\begin{center}
    \large
    {\Large Measuring Justice in Machine Learning\\}
\vspace{4mm}
    {by\\}
\vspace{4mm}
    {Alan Lundgard\\}
\vspace{4mm}
    {Submitted to the Department of Electrical Engineering and Computer Science\\in Partial Fulfillment of the Requirements for the Degree of\\}
\vspace{4mm}
    {Master of Science in Computer Science and Engineering\\}
    {at the\\}
    {Massachusetts Institute of Technology\\}
\vspace{4mm}
    {September 2020\\}
\end{center}

\begin{flushleft}
\Large
Abstract
\end{flushleft}

\noindent
How can we build more just machine learning systems? To answer this question, we need to know both what justice is and how to tell whether one system is more or less just than another. That is, we need both a definition and a measure of justice. Theories of distributive justice hold that justice can be measured (in part) in terms of the fair distribution of benefits and burdens across people in society. Recently, the field known as fair machine learning has turned to John Rawls’s theory of distributive justice for inspiration and operationalization. However, philosophers known as capability theorists have long argued that Rawls’s theory uses the wrong measure of justice, thereby encoding biases against people with disabilities. If these theorists are right, is it possible to operationalize Rawls’s theory in machine learning systems without also encoding its biases? In this paper, I draw on examples from fair machine learning to suggest that the answer to this question is no: the capability theorists’ arguments against Rawls’s theory carry over into machine learning systems. But capability theorists don’t only argue that Rawls’s theory uses the wrong measure, they also offer an alternative measure. Which measure of justice is right? And has fair machine learning been using the wrong one?

\begin{flushleft}
    {Thesis Supervisor: Arvind Satyanarayan\\}
    {Title: Assistant Professor of Electrical Engineering and Computer Science\\}
\end{flushleft}

\begin{flushleft}
    {Thesis Co-Supervisor: Sally Haslanger\\}
    {Title: Ford Professor of Philosophy\\}
\end{flushleft}

\begin{flushleft}
    {Thesis Reader: Reuben Binns\\}
    {Title: Associate Professor of Human Centered Computing\\}
\end{flushleft}

==> _titlepage.tex <==
\thispagestyle{empty}
\begin{center}
    \large
    {\Large Measuring Justice in Machine Learning\\}
\vspace{4mm}
    {by\\}
\vspace{4mm}
    {Alan Lundgard\\}
\vspace{4mm}
    {B.S., University of Michigan, Ann Arbor, 2017\\}
\vspace{4mm}
    {Submitted to the Department of Electrical Engineering and Computer Science\\in Partial Fulfillment of the Requirements for the Degree of\\}
\vspace{4mm}
    {Master of Science in Computer Science and Engineering\\}
    {at the\\}
    {Massachusetts Institute of Technology\\}
\vspace{4mm}
    {September 2020\\}
\vspace{4mm}
    {\large \copyright Alan Lundgard. All rights reserved.\\}
\vspace{4mm}
    {\large
        The author hereby grants to MIT permission to reproduce\\and to distribute publicly paper and electronic copies\\of this thesis document in whole or in part\\in any medium now known or hereafter created.
    \\}
\vspace{4mm}
\end{center}

{\large
\begin{flushleft}
    {Author \dotfill}
\end{flushleft}
\vspace{-6mm}
\begin{flushright}
    {Department of Electrical Engineering and Computer Science\\}
    {August 28, 2020\\}
\end{flushright}

\begin{flushleft}
    {Certified by \dotfill}
\end{flushleft}
\vspace{-6mm}
\begin{flushright}
    {Arvind Satyanarayan\\}
    {Assistant Professor of Electrical Engineering and Computer Science\\}
    {Thesis Supervisor}
\end{flushright}

\begin{flushleft}
    {Certified by \dotfill}
\end{flushleft}
\vspace{-6mm}
\begin{flushright}
    {Sally Haslanger\\}
    {Ford Professor of Philosophy\\}
    {Thesis Co-Supervisor}
\end{flushright}

\begin{flushleft}
    {Certified by \dotfill}
\end{flushleft}
\vspace{-6mm}
\begin{flushright}
    {Reuben Binns\\}
    {Associate Professor of Human Centered Computing\\}
    {Thesis Reader}
\end{flushright}

\begin{flushleft}
    {Accepted by \dotfill}
\end{flushleft}
\vspace{-6mm}
\begin{flushright}
    {Leslie A. Kolodziejski\\}
    {Professor of Electrical Engineering and Computer Science\\}
    {Chair, Department Committee on Graduate Students\\}
\end{flushright}
}

